Deep Learning for Time Series Forecasting: The Electric Load Case

Management and efficient operations in critical infrastructure such as Smart Grids take huge advantage of accurate power load forecasting which, due to its nonlinear nature, remains a challenging task. Recently, deep learning has emerged in the machine learning field achieving impressive performance in a vast range of tasks, from image classification to machine translation. Applications of deep learning models to the electric load forecasting problem are gaining interest among researchers as well as the industry, but a comprehensive and sound comparison among different architectures is not yet available in the literature. This work aims at filling the gap by reviewing and experimentally evaluating on two real-world datasets the most recent trends in electric load forecasting, by contrasting deep learning architectures on short term forecast (one day ahead prediction). Specifically, we focus on feedforward and recurrent neural networks, sequence to sequence models and temporal convolutional neural networks along with architectural variants, which are known in the signal processing community but are novel to the load forecasting one.

==> sections/datasets.tex <==
\section{Datasets}
\label{sec:datasets}

\subsection{\uci}
The \uci (\ucishort) contains 2075259 measurements of electric power consumption in one household located in Sceaux (7km of Paris, France) between December 2006 and November 2010 (47 months) with a one-minute sampling rate. Different electrical quantities and some sub-metering values are available but in this study we focus on prediction of the "Global active power".
All calendar timestamps are present in the dataset but some measurement values are missing (nearly 1,25\% of the values). We impute the missing values with the mean power consumption for the corresponding hour and minute across the different years of measurements. 
In this study the dataset has been re-sampled using a sampling rate of 15 minute which is more common in smart meters technologies.
For this task we decide to do not include any exogenous variable but to perform the forecasting using only historical load values.  
% We study the seasonality pattern in the \ucishort dataset by observing the autocorrelation function computed for a sufficient number of lags, such that hourly, daily or weekly patterns (if any) can be observed. On the left-side of Figure \ref{fig:uci_af} the autocorrelation function up to 1440 lag is depicted, and a major seasonality pattern at lag 96 (one day) and a minor one at 48 (half-day) are easily identifiable. In order to remove the seasonality we apply a differentiation at lag 96. Notice that by taking this first differentiation we have to discard the last day of measurements (i.e the last 96 timesteps).
% The right-side in Figure \ref{fig:uci_af}) depicts the autocorrelation function of the newly obtained data, as can be observed both the minor and major personalities has been removed and a new cyclic pattern appears at lag 672 (a week). Similarly to \cite{RNN_Bianchi} we decide to do not proceed with a further differentiation in order to do not waste too many observation points. 
Figure \ref{fig:uci} depicts the average daily and weekly electric consumption, as one can expect the highest consumption values are registered in the morning and in the evening, when most of the people are in their houses. Moreover, the average load profile over a week clearly shows how weekdays are similar in terms of trends while weekends present generally higher consumption. 
In the figures we can notice that the data are characterized by high variance, thus in order to stabilize it we apply a log transformation to them.
This task consist in forecasting the electric load for the next day, i.e. 96 steps ahead. The performances of the models on the last year of measurements provides us with a comparable quantity of their generalization capabilities, we will refer to this data points as the test set. The remaining measurements are repeatedly divided in two sets, holding out a month of data every five. This process allows us to build a training set and a validation set where different hyper-parameters configurations can be evaluated. Only the best performing configuration is later evaluated on the test set.

% \begin{figure*}
% \begin{multicols}{2}
%     \includegraphics[width=\linewidth]{img/uci/uci_acf1.png}\par 
%     \includegraphics[width=\linewidth]{img/uci/uci_acf_diff_lag96_1.png}\par
% 	\end{multicols}
% \label{fig:uci_af}
% \caption{On the left-side the autocorrelation function for the \ucishort dataset. On the right-side the autocorrelation function after a seasonal differentiation (96 lag).}
% \end{figure*}

\begin{figure}
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{img/uci/uci_D.png}\par 
    \includegraphics[width=\linewidth]{img/uci/uci_D_quantiles.png}\par 
    \end{multicols}
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{img/uci/uci_W.png}\par
    \includegraphics[width=\linewidth]{img/uci/uci_W_quantiles.png}\par
	\end{multicols}
\label{fig:uci}
\caption{Daily (top) and weekly (bottom) statistics for the for the active power in the whole \ucishort. On the left-side, mean, median and standard deviation. On the right-side the green area represent the quantiles Q1 to Q3.}
\end{figure}

\subsection{\gc}
The \gcshort dataset \cite{GEFCom2014} was made available on CrowdANALYTIX for an online forecasting competition that lasted between August 2015 and December 2015. The dataset contains 60600 measurements of electric power consumption collected by ISO New England between January 2005 and December 2011 with a one-hour sampling rate. Differently from the \ucishort dataset, temperature values are also available and will be used by the models to enhance their predictive capabilities. In particular the input variables being used for forecasting the next $\outlen$ at timestep $t$ include: several previous load measurements $\ell^{(t-1)}, \dots, \ell^{(t-\inlen)}$, the temperature measurements for the previous timestep registered by 25 different stations $T^{(t-1)}_1, \dots, T^{(t-1)}_{25}$, hour, day, month and year are also provided.
We did apply standard normalization to load and temperature measurements while for the categorical variables we simply apply one-hot encoding.
In Figure \ref{fig:gc} we can observe the average load and the data dispersion on a daily and weekly basis.  Compared to \ucishort, the load profiles looks much more regular. This observation is quite natural because the load measurements from the previous dataset comes from a single household, thus the stochasticity introduced by user behaviour is much more visible there. On the opposite, the load information in \gcshort comes from an aggregation of the data coming from several different smart meters which, overall, exhibits a more stable and regular pattern.
This task, like the previous one, consists in forecasting the electric load for the next day, i.e. 24 steps ahead. The hyper-parameters optimization and the final score for the models follow the same guidelines provided for \ucishort.

\begin{figure}
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{img/gefcom/gefcom_D_std.png}\par 
    \includegraphics[width=\linewidth]{img/gefcom/gefcom_D_q.png}\par 
    \end{multicols}
\begin{multicols}{2}
    \includegraphics[width=\linewidth]{img/gefcom/gefcom_W_std.png}\par 
    \includegraphics[width=\linewidth]{img/gefcom/gefcom_W_q.png}\par 
	\end{multicols}
\label{fig:gc}
\caption{Daily (top) and weekly (bottom) statistics for the for the electric load in the whole \gcshort dataset. On the left-side, mean, median and standard deviation. On the right-side the green area represent the quantiles Q1 to Q3.}
\end{figure}

==> sections/results.tex <==
\section{Results}
